Optimal Baseline Corrections for Off-Policy Contextual Bandits

The off-policy learning paradigm allows for recommender systems and general ranking applications to be framed as decision-making problems, where we aim to learn decision policies that optimize an unbiased offline estimate of an online reward metric. With unbiasedness comes potentially high variance, and prevalent methods exist to reduce estimation variance. These methods typically make use of control variates, either additive (i.e., baseline corrections or doubly robust methods) or multiplicative (i.e., self-normalisation). Our work unifies these approaches by proposing a single framework built on their equivalence in learning scenarios. The foundation of our framework is the derivation of an equivalent baseline correction for all of the existing control variates. Consequently, our framework enables us to characterize the variance-optimal unbiased estimator and provide a closed-form solution for it. This optimal estimator brings significantly improved performance in both evaluation and learning, and minimizes data requirements. Empirical observations corroborate our theoretical findings.

==> sections/Discussion.tex <==
%%%%%%%%%%%%%%%%%%%%
%% All discussions b/w OJ and SG.
% \appendix
% \section{On Gradients and Log-tricks}
% \oj{I've never fully understood why you need REINFORCE, I guess? Trying to understand it better}

% Take an on-policy objective:
% \begin{equation}
% \begin{split}    
%     V(\pi) = \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi(\cdot|x)}\mleft[ r(a,x) \mright]\mright].
% \end{split}
% \end{equation}

% If this is the objective, then the ''true''/''unbiased'' gradient for the objective would be:

% \begin{equation}
% \begin{split}    
%    \nabla V(\pi) = \nabla \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi(\cdot|x)}\mleft[ r(a,x) \mright]\mright].
% \end{split}
% \end{equation}

% We cannot take the gradient term inside the expectations, because the second expectation depends on the policy itself. Replacing the inner expectation with the sum over all actions.

% \begin{equation}
% \begin{split}    
%    \nabla V(\pi) &= \nabla \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[ \sum_{a} \pi(a|x) \mleft[ r(a,x) \mright]\mright], \\
%     &= \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[ \sum_{a} \nabla \pi(a|x) \mleft[ r(a,x) \mright]\mright], \\
%     &= \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[ \sum_{a}  \pi(a|x) \nabla \log \pi(a|x) \mleft[ r(a,x) \mright]\mright], \\
%     &= \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[ \sum_{a}  \pi(a|x) \nabla \log \pi(a|x) \mleft[ r(a,x) \mright]\mright], \\
%     &= \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[ \mathop{\mathbb{E}}_{a \sim \pi(\cdot|x)}  \nabla \log \pi(a|x) \mleft[ r(a,x) \mright]\mright], \\
% \end{split}
% \end{equation}

% Now you can take a sample estimate of the gradient above, to get a ''sample'' gradient for the on-policy objective:

% \begin{equation}
% \nabla \widehat{V}(\pi, \mathcal{D})  = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \nabla \log \pi(a|x) \cdot r.
% \end{equation}

% \sg{This is an unbiased gradient estimate of the ''true'' gradient estimate of the on-policy objective}

% With the Importance Sampling trick, we replace the following estimator:

% \begin{equation}
%      \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot|x)}\mleft[ \frac{\pi(a|x)}{\pi_{0}(a|x)} R \mright]\mright].
% \end{equation}
% with sampled action, context, i.e. we replace the expectation $\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot|x)}$  with the sample/logged actions $a_i$, we get the following sample estimate for the case of IPS:

% \begin{equation}
%     \widehat{V}_{\rm IPS}(\pi,\mathcal{D}) = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a|x)}{\pi_{0}(a|x)} r.
% \end{equation}

% We have the policy term with IPS, because  it is inside the in expectation over $\pi_{0}$. 

% Now with this off-policy IPS objective, we don't really need the log-derivative trick, since we can directly take the gradient inside the summation, but still it's used in off-policy learning papers~\cite{chen2019top,ma2020off} I guess to be consistent with the RL literature?

% \sg{--- SG's comment ends. Does this make sense?. Please correct me if I am wrong :) --}


% \oj{This is wrong:}
% Take a sample estimate (of on-policy objective):
% \begin{equation}
% \widehat{V}(\pi, \mathcal{D})  = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \pi(a|x) \cdot r.
% \end{equation}

% \sg{Stupid question, but wouldn't the sample estimate of Eq. 36 be just average $ \frac{1}{N} \sum_{i} r(x_i, a_i)$ across the samples? i.e. just the average of the rewards for the sampled actions and contexts. For ex: the sample estimate of the quantity $\mathbb{E}_{x\sim\mathsf{P}(X)} (f(x))$ is just $ \frac{1}{N} \sum_{i, x_i \sim \mathsf{P}(X)} f(x_i)$.}
% \oj{Not a stupid question: thank you for correcting me. I messed up here and was wrong! Updating so it makes sense.}

% \oj{Updating so things make sense:}

% We can write expand the expectation in $V(\pi)$ to get:
% \begin{equation}
% \begin{split}    
%     V(\pi) = \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[\sum_{a \in \mathcal{A}}\mleft[  \pi(a|x)\cdot r(a,x) \mright]\mright].
% \end{split}
% \end{equation}

% Naturally, we cannot compute this from a sample estimate because we do not know $r(a,x)$ for ``counterfactual'' actions.
% So suppose we have a model $\widehat{r}(a,x)$ instead. Now we recover the Diret Method:

% \begin{equation}
%     \widehat{V}_{\rm DM}(\pi, \mathcal{D}) = \frac{1}{\mathcal{D}} \sum_{x \in \mathcal{D}}\sum_{a \in \mathcal{A}}\pi(a|x)\cdot r(a,x).
% \end{equation}



% % Maximise this via gradient descent. The gradient:

% % \begin{equation}
% % \nabla_{\pi} \widehat{V}(\pi, \mathcal{D})  = \nabla_{\pi} \mleft(\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \pi(a|x) \cdot r \mright).
% % \end{equation}

% % This is a quantity we can simply compute, right?
% % Why do we need policy gradients and/or log-tricks?

% % In any case, the log-trick means we instead compute:
% % \begin{equation}
% % \nabla_{\pi} \widehat{V}(\pi, \mathcal{D})  = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \pi(a|x) \cdot r \cdot \nabla_{\pi} \log(\pi(a|x)) .
% % \end{equation}

% There are loads of online ``tutorials'' implementing the ``log-trick'' in PyTorch via these two lines of code:


% \texttt{loss = log(policy.log\_prob(action)) * reward}

% \texttt{loss.backward()}

% Isn't this very wrong? Now you're instead optimising this estimator:
% \begin{equation}
% \widehat{V}(\pi, \mathcal{D})  = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \log(\pi(a|x)) \cdot r.
% \end{equation}

% These are not equivalent!

% \sg{I think the correct way to implement the ''log-derivative'' trick in our case would be:}

% \texttt{loss = (policy.prob(action).detach() * policy.log\_prob(action) * reward}

% \texttt{loss.backward()}

% The ''detach()'' function will remove the $\pi(a|x)$ part from the gradient computation, and only flow the gradient to the log-policy part. I think this operation is called as ''stop-gradient'' in tensorflow. 

% This shows an equivalence to Eq.~\ref{eq:MC_gradient_IPS}; the connection between SNIPS and the REINFORCE baseline correction is well-known, but seldom mentioned or explored in the research literature.
% Whereas baseline corrections were introduced to combat gradient variance during on-policy learning, SNIPS and BanditNet construct a variance-reduced equivariant objective for off-policy learning and evaluation.

% To summarise: self-normalisation of the objective function can equivalently be achieved by an (a priori unknown) translation on the logged rewards, which is then equivalent to the common variance reduction technique of ``\emph{baselining}'' gradient estimates.

% \oj{Does it make sense to compare the variance of the IPS gradient with the optimal baseline to that of the SNIPS gradient (instead of BanditNet)? \cite[Eq. 8]{Swaminathan2015} (or \cite[Eq. 9.9]{Owen2013}) gives an estimator for SNIPS variance, we could adapt it to get SNIPS' \emph{gradient} variance}

% \sg{That's a good idea. But do people use SNIPS for off-policy learning? From what I remember from the BanditNet paper, an unbiased mini-batch (stochastic) gradient for SNIPS does not exist \cite[Appendix C]{Joachims2018}. But we could cite this and then only compare the variance with the BanditNet gradient. From the face of it, since the optimal baseline is the minimum of the variance of the gradient, any other baseline method (including BanditNet) should be worse off than this, right?}

% \oj{I'm currently working on something where we do Norm-POEM (essentially SNIPS with variance regularisation). But because it's full-batch optimisation, I guess gradient variance does not matter as much... Agreed that the optimal baseline should improve over BanditNet though.}
% \sg{Is Norm-POEM optimized using full-batch gradient descent? (I have not used it so not sure.) If so, then how can it scale to large-scale production logged data in real life application?}
% \oj{It does not :D you use relatively small data and relatively big servers. Their original paper uses LBFGS.}
% \sg{Got it, thanks :)}

% \oj{What's below (until \S \ref{sec:ranking_OPE}) is under construction.}
% The gradient of the SNIPS estimator is given by:

% \begin{align}
%    \nabla V_{\rm SNIPS} &= \nabla \mleft(\frac{\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}} r]}{\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}]}\mright)\nonumber\\
%    &= \frac{\nabla\mleft(\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}} r]\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}]\mright) + \mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}r]\nabla\mleft(\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}]\mright)}{\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}]^{2}} \nonumber\\
%    &= \frac{2\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}} r] \nabla \mleft(\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}]\mright) + \mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}] \nabla \mleft(\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}} r]\mright) }{\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}]^{2}} \nonumber \\
%    &= \frac{2\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}} r] \mathbb{E}[\frac{\nabla\pi_{\theta}}{\pi_{0}}] + \mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}] \mathbb{E}[\frac{\nabla \pi_{\theta}}{\pi_{0}} r]}{\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}]^{2}} \nonumber \\
%   % &= 2\mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}} r] \mathbb{E}[\frac{\nabla\pi_{\theta}}{\pi_{0}}] + \mathbb{E}[\frac{\pi_{\theta}}{\pi_{0}}] \mathbb{E}[\frac{\nabla \pi_{\theta}}{\pi_{0}} r] \nonumber \\
% \end{align}
% %
% \sg{Thanks for writing the gradient for SNIPS. I was wondering if we write the gradient in terms of the 
% "true" expectations (as opposed to sample estimates) of the individual terms, the gradient of the denominator of the original SNIPS estimator is zero, and the expected value of the importance sampling ratio (denominator) is exactly 1, so the gradient of the SNIPS estimator reduces to the gradient of the IPS estimator.}
% %
% \begin{align}
%     \mathbb{E}[\frac{\nabla \pi_{\theta}}{\pi_{0}}] 
%    &= \nabla \mathbb{E}[\frac{ \pi_{\theta}}{\pi_{0}}] \\
%    &= \nabla \sum_{a}^{} \pi_0(a \mid x) \frac{ \pi_{\theta} (a \mid x)}{\pi_{0}(a \mid x)} \\
%    &= \nabla  \sum_{a}^{}  \pi_{\theta} (a \mid x) \\
%    &= \nabla 1 = 0
% \end{align}
% %
% \begin{align}
%     \mathbb{E}[\frac{ \pi_{\theta}}{\pi_{0}}] 
%    &=  \sum_{a}^{} \pi_0(a \mid x) \frac{ \pi_{\theta} (a \mid x)}{\pi_{0}(a \mid x)} \\
%    &= 1
% \end{align}
% \sg{Is my reasoning correct? I think we should try to analytically get the variance of the sample estimate of the SNIPS estimator? What do you think? For the IPS estimator, calculating the variance of the sample gradient estimate does not change the analysis (from what we have right now), since we will only have an additional constant $N$ term for the variance of the sample estimator for IPS, and from Eq. 19 it cancels out (along with a constant 2). }
% \sg{I changed the variance of the sample estimate of the objectives (on-policy and off-policy both, as opposed to the variance of the true objective. I changed it in the previous sections, let me know if you disagree.}
% \oj{What an awesome thing to wake up to! I had the same thought when the SNIPS gradient started to cancel out, stopped updating this and closed my laptop then, thinking ``tomorrow I should probably consider the sample estimate''. Will check whether your derivation is correct but I'm guessing it probably is, thanks Shashank!}
% \sg{That's great to know :)}

%where $b$ is the baseline correction term to reduce the variance. 
%A simple choice for the baseline $\beta$ could be the average reward across the current mini-batch $\mathcal{B}$.
%In practice, 
%\sg{Does this make sense? If this is a valid baseline correction, then the gradient looks very similar to the BanditNet objective gradient.}

% \oj{Theorem 4 in \href{https://proceedings.neurips.cc/paper_files/paper/2001/file/584b98aac2dddf59ee2cf19ca4ccb75e-Paper.pdf}{this paper}~\cite{Greensmith2004} shows the optimal baseline correction, can we translate it to our notation? Thorsten writes in BanditNet: ``\emph{we cannot sample new roll-outs from the current policy under consideration, which means we cannot use the standard variance-optimal estimator used in REINFORCE}''. Is this relevant for us? Can we use similar results to derive optimal baselines?}

% \sg{Good point. This is indeed relevant for our setup. I will write down the variance optimal baseline for the on-policy bandit setup. But I don't agree with Thorsten's statement in the BanditNet paper. We can derive a similar variance optimal baseline correction for off-policy bandits. I derived it similar to the on-policy case, I will add it to latex. But I am not sure of it's connection with the SNIPS estimator.}

% \oj{Thank you! About connection with SNIPS: if we call the optimal baseline $\lambda^{\star}$, it'd be interesting to look at $S^{\star}$ (and SNIPS) as a function of $\lambda^{\star}$}

%

% \sg{A random idea: What if we use the running average $\sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a|x)}{\pi_{0}(a|x)}$ (running average IS ratio across mini-batches batch) as baseline, then is it equivalent to optimizing for the SNIPS objective?}


% \sg{Does this make sense? Need to double check the derivation.} \oj{Awesome! Added a version to the plot that uses this sample estimate i.s.o. the grid search. I guess you could in practice simply: compute the estimated optimal baseline, compute the variance you get with this estimated optimal baseline, if it's higher than SNIPS use SNIPS instead... In this way, you don't lose SNIPS' advantage of having no tuneable hyperparameters, and get the best of both worlds}
% \sg{That's an excellent idea. We could write it in a single expression I suppose, with an indicator function which activates SNIPS or $\beta$-IPS based on the empirical variance of the two estimators. A similar estimator was proposed in an older paper~\cite{wang2017optimal}. }

%\subsubsection{Gradient Estimation for Off-Policy Bandits}

% \oj{I messed up somewhere (looks like the above just gives SNIPS again?), might be too late on a Friday for me to push this over the line}

% \oj{OK, I thought it was weird ( and don't think I fully grasp it yet), but the SNIPS estimator is essentially the same thing as doing a baseline correction with *drum roll* the SNIPS estimator itself.}
% \sg{Wow, that's interesting, I need to look closer to understand it, but great catch :)}

% \oj{Come to think of it, it probably comes from the fact that SNIPS is equivariant to translations in the reward...}

% \oj{Note: Eq.\ref{eq:optimal_offpolicy_beta} behaves strangely when $\pi \approx \pi0$?}
% \sg{Maybe we need a clipping operation here? To avoid a $0$ in the denominator}

% \oj{In cases this estimate does not work well (or does not behave nicely), we could still simply do gradient descent on the variance to obtain $\beta$ (i.e. exactly what ~\citeauthor{Farajtabar2018} propose~\cite{Farajtabar2018}).}

% \oj{This is essentially doing doubly robust with a constant reward estimate $\beta$, and so it's simply an additive control variate compared to the multiplicative variate we have in SNIPS. This even creates a nice connection to Harrie's recent work on doubly-robust estimation for rankings.}
% \sg{Agreed! And the gradient of this estimator is same as the gradient for IPS with baseline correction, so there's a nice connection there as well.}
% \sg{We probably need to read some theoritical off-policy estimator paper which analyses properties of any given estimator. If we can then do similar analysis with this estimator, then it seems like a great contribution.}

% \oj{Genuine question: do people actually use this when doing off-policy evaluation with IPS? If the answer is no, why? The fact that it outperforms SNIPS is quite surprising to me! Might be the example, but still.}

% \sg{I am not really sure honestly. This seems like a good idea in principle. We can probably check the theoritical properties of this estimator, and compare against the ones used in practice. I am not well versed with off-policy bandit estimator's latest advancements. There seems to be some work from Thorsten on this~\cite{su2020doubly}. Practically speaking, you don't need to fit a regression model with this estimator, so it's easy to use as compared to the DR estimator.}

% \oj{I think it's even more closely related to the ``More Robust Doubly Robust'' approach~\cite{Farajtabar2018}, where they learn the regression model in DR that minimises the variance of the resulting DR estimator. }

%%%%%% OJ - SG discussion
% \sg{We need to estimate $\pi(a_{k}|x, j)$ in both IIPM and PBM click model, right? It involves an expectation over the rankings sampled from $\pi$, so we need to use the log-derivative (REINFORCE) trick here.}
% \oj{Aha, are these propensities typically estimated using Monte Carlo sampling?
% I (having never used this stuff in practice) assumed you would find a way to get an analytical expression for  $\pi(a|x, k)$ and plug that in.}
% \sg{Right, we need sampling to estimate the propensities. To estimate the propensity under the logging policy (the denominator term), in practice, it's usually a mix of monte-carlo sampling and exploiting the Plackett-luce model structure (assuming the policy is modelled as a PL). Generally, there are two ways to estimate the logging propensity: 1) You can "query" the logging policy model ($\pi_0$) to sample additional $N$ rankings per query, and then use Monte-carlo sampling, or 2) You can use the logged data to estimate it. I personally use the second method, with the assumption that we only have access to the logged data in practice. For the propensity under the new policy (the numerator term), we can use REINFORCE (or PL-rank from Harrie) to get the gradient of the IPS objective followed by a monte-carlo sampling to replace the expectation term. \url{https://arxiv.org/pdf/1911.08054.pdf} Eq 13 in this paper has an easy to understand REINFORCE gradient term for the PBM IPS objective.}
% \oj{Ben's SNIPM paper does things slightly differently~\cite[\S B.1]{London2023}: they use some sort of Fisher-Yates variant to get an analytical expression for the propensities. There's probably an advantage to both approaches (yours is more general, theirs is restrictive but efficient). Could be interesting to consider.}
% \sg{I see. The Fisher-Yates algorithm is essentially doing random interventions in the ranking to get a closed-form expression for the logging propensity. But this is only valid for the logging propensity; for the new policy $\pi$, can we do something similar (offline)? Not sure. I am curious about this part though. Can we use a softmax policy with IPM (or PBM) model instead of a Plackett-luce model? Can we optimize the IPM/PBM objective without applying REINFORCE?}

% \sg{I tried to derive the optimal baseline for the PBM model, but the problem with the PBM model is that the denominator is a constant w.r.t. to the logging policy (since we are marginalizing it out), and the variance of the gradient has no baseline term. }
% \newline
% \sg{Perhaps for this work, we can just focus on the IPM click model? IPM click model was also used in a recent top-K off-policy KDD paper: \url{https://www.csie.ntu.edu.tw/~cjlin/papers/counterfactual_topk/xcf.pdf}? And leave the optimal baseline for PBM for a future work? If we come up with an optimal baseline for the IPM click model, that could be a good contribution in itself?}
% \oj{Agreed! Still an interesting problem, but it looks like we're honing in on a contribution that would already be valuable.}
% \sg{A practical question: At Instagram or ShareChat scale (millions/billions of items), how do you estimate the second sum in Eq. 20 efficiently? (given that it sums over \emph{all} items in the action space (corpus)). To me it looks like an expectation of $\hat{r}$ w.r.t. $\pi$, so maybe one can apply REINFORCE trick here, by monte-carlo sampling few items from $\pi$, and then using log-derivative trick? (for computing the gradient of the term)}

% \oj{Exactly as you say, you sample. We do this for continuous action spaces (real-time-bidding in \cite{Jeunen2023_AuctionGym}). Another thing is that this simplifies massively for deterministic target policies, of course. I think in general, people never use this stuff for the full action space of all available items, but smaller-scale problems instead. The size of the action space is always the core driver of variance.}
% \sg{Thanks! This makes sense, good to know this.}

% \sg{Q: Are we assuming the reward distribution to be a constant? $P(R=r \mid x,a)$ Asking this because existing variance analysis for IPS also consider the mean and variance of the reward distribution~\cite{wan2022safe}, and the expressions are generally more involved~\cite{Dudik2014} (Theorm 2), so I was wondering. But the proposed methods use "estimated" logging propensity instead of the "actual" propensity, so maybe that's why their analysis is more complicated than ours?}

% \oj{Only if we have to, I'd say? If we don't have to limit ourselves, let's not.}

% \sg{Sure. I am reading variance analysis in existing papers for IPS (ex: \cite{wan2022safe}), and they include reward mean and variance in their expression, so I got a bit confused. I will read some more off-policy bandit papers carefully w.r.t. their variance analysis (ex: \cite{tucker2023variance}), just to be sure. I will also discuss this with Harrie.}

% \sg{Sorry for the long comment, just writing out my thoughts.}

% \oj{Sure! Which equation/derivation do you think might be missing a term for the reward variance?  }

% \sg{I think the off-policy derivations. We have 3 rando variables ($x, a, r$) which can make the analysis more complicated, and I got confused with different equations used in other papers. But if we use the "true" propensities, the derivations will hold. I will check variance analysis with multiple random variables in general, just to be sure.}

% \oj{OK, thanks! I'm used to working with known ``true'' propensities, so I think we can keep that assumption if it simplifies the analysis}



%%%%%%%%%%%




%%%%%%%%%%%%% LTR 

% \section{Learning-to-Rank}
% \subsection{Off-Policy Estimation for Rankings}\label{sec:ranking_OPE}
% The general off-policy estimation setup introduced in Section~\ref{sec:general_OPE} is widely applicable to a swath of general use-cases, from pure recommendation~\cite{Jeunen2020} to ad-load balancing~\cite{Sagtani2023} and real-time bidding~\cite{Jeunen2023_AuctionGym}.
% Nevertheless, in \emph{ranking} applications we typically require additional assumptions to make the problem tractable.
% Indeed, treating every possible ranking as an atomic action leads to a combinatorial explosion of the action space that quickly renders effective off-policy estimation \emph{in}tractable due to excessive variance in the proposed estimators.
% For a list of assumptions that are necessary to motivate the widely used Discounted Cumulative Gain (DCG) metric in this off-policy estimation framework, see~\citeauthor{Jeunen2023_nDCG}~\cite{Jeunen2023_nDCG}.
% We adopt several of the assumptions they lay out to allow for tractable counterfactual estimation: independence of item-level rewards within rankings and independence of rewards across user sessions.

% For an excellent overview of typical \emph{click} models~\cite{Chuklin2015} being leveraged in conjunction with the classical IPS estimator, see~\citeauthor{Li2018}~\cite{Li2018}.

% We now extend our mathematical notation to include ranking setups.
% An action $a$ will now refer to a ranking of items rather than a single item, where $a_{k}$ denotes the $k$\textsuperscript{th} item in the ranking.
% Rewards are also observed at an item-level, and $r_{k}$ analogously refers to the observed reward at rank $k$.
% $L \equiv |a|$ is the length of the ranked list.

% Propensities are now: $\pi(a|x,k) \equiv \mathsf{P}(A=a|X=x,K=k,\Pi=\pi)$.

% \subsubsection{Item-Position Model (IPM)}
% Assume that the probability of observing a reward for an item $a$ at position $k$ only depends on the item and the position.
% Through the same importance sampling trick as for $\widehat{V}_{\rm IPS}$, we can formulate the IPM estimator:
% \begin{equation}\label{eq:IPM}
%     \widehat{V}_{\rm IPM}(\pi,\mathcal{D}) = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} r_{k}.
% \end{equation}
% Note that this formulation appears i.a. in the work of \citeauthor{London2023}~\cite{London2023}, whereas \citeauthor{Li2018}~\cite{Li2018} denote propensities as $\pi(a_{k}, k|x)$ instead.
% It is fairly easy to see that these forms are equivalent, because of a normalising constant. Indeed, via Bayes' rule we have:
% \begin{equation}
% %    \mathsf{P}(A|B,C) = \frac{\mathsf{P}(A,B|C)}{\mathsf{P}(B|C)}
%     \pi(a_{k}|x,k) = \frac{\pi(a_{k}, k|x)}{\mathsf{P}(K=k|X=x)}.
% \end{equation}
% Because $\mathsf{P}(K=k|X=x)$ is a constant that appears in both the numerator and the denominator of the importance weights, it cancels.

% The gradient for Eq.~\ref{eq:IPM} with respect to the policy parameters, with baseline correction $\beta$, is straightforwardly derived to be:
% \begin{equation}\label{eq:MC_gradient_IPM}
%     \nabla \widehat{V}_{\rm IPM}(\pi, \beta, \mathcal{B}) = \frac{1}{\mleft|\mathcal{B}\mright|} \sum_{(x,a,r) \in \mathcal{B}} \sum_{k=1}^{L} \frac{\nabla\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} (r_{k}-\beta).
% \end{equation}


% The global optimal baseline for the IPM click model is given as:
% %
% \begin{equation}\label{eq:optimal_offpolicy}
%     \beta^{*} = \frac{ \sum_{k=1}^{L} \mathop{\mathbb{E}}\mleft[ \frac{ \| \nabla \pi(a_k|x,k))\|^2_2}{\pi_{0}(a_k|x,k)^2} r_k \mright]}{ \sum_{k=1}^{L} \mathop{\mathbb{E}}\mleft[  \frac{ \| \nabla \pi(a_k|x,k))\|^2_2}{\pi_{0}(a_k|x,k)^2} \mright]}
% \end{equation}

% Similarly, we can derive a local, per-rank baseline for the IPM click model, which is given by:
% %
% \begin{equation}\label{eq:optimal_offpolicy}
%     \beta_k^{*} = \frac{  \mathop{\mathbb{E}}\mleft[ \frac{ \| \nabla \pi(a_k|x,k))\|^2_2}{\pi_{0}(a_k|x,k)^2} r_k \mright]}{ \mathop{\mathbb{E}}\mleft[  \frac{ \| \nabla \pi(a_k|x,k))\|^2_2}{\pi_{0}(a_k|x,k)^2} \mright]}
% \end{equation}

% \citeauthor{London2023} propose methods that allow for self-normalised IPS weighting in the IPM~\cite{London2023}, with both a \emph{local} variant that uses a control variate per position $k$, and a \emph{global} variant that utilises a single control variate.
% Analogous to the SNIPS control variate given by Eq.~\ref{eq:control_variate}, the SNIPM control variate for a fixed position $k$ is proposed as the average importance weight:
% \begin{equation}\label{eq:control_variate_ipm_local}
%    \mathop{\mathbb{E}}_{(x,a,r) \sim \mathsf{P}(X,A,R|\Pi=\pi)}\mleft[
%    \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)}
%    \mright] = 1.
% \end{equation}
% This gives rise to the SNIPM estimator with $k$ \emph{local} control variates:
% \begin{equation}
%     \widehat{V}_{\rm SNIPM}(\pi,\mathcal{D}) =  \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} r_{k}}{\sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)}}.
% \end{equation}
% It is easily verified that the expectation still equals 1 when averaged over all positions $1\leq k \leq L$, justifying the SNIPM estimator with a single \emph{global} control variate:
% \begin{gather}\label{eq:control_variate_ipm_global}
%    \mathop{\mathbb{E}}_{(x,a,r) \sim \mathsf{P}(X,A,R|\Pi=\pi)}\mleft[
%    \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)}
%    \mright] = 1,\\
% %\end{equation}
% %\begin{equation}
%     \widehat{V}_{\rm SNIPM-G}(\pi,\mathcal{D}) =  \frac{\sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} r_{k}}{\sum_{(x,a,r) \in \mathcal{D}} \frac{1}{L}\sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)}}.
% \end{gather}

% Similarly to SNIPS, SNIPM(-G) do not decompose into a single sum over observed samples, which complicates mini-batch optimisation. A similar reduction from self-normalisation to a translation on the reward would solve this, but is absent from the research literature so far.
% We derive this in Section~\ref{sec:SNIPM_reward_translation}.

% % It is easily verified that this equation still holds for a fixed position $k$, justifying the SNIPM estimator with a \emph{local} control variate:
% % \begin{equation}
% %     \widehat{V}_{\rm SNIPM}(\pi,\mathcal{D}) =  \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} r_{k}}{\sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)}}.
% % \end{equation}
% % From this, we can also define the \emph{global} SNIPM estimator:

% \subsubsection{Position-Based Model (PBM)}
% The IPM does not make strong assumptions w.r.t. position bias. 
% This ensures its general applicability, but implies that its variance will be excessive in cases where we can deduce further structure in user behaviour with rankings.
% Intuitively: the IPM does not allow signal to be shared across positions.
% That is, if an item $a$ yields a reward at rank $k$, we have no way to infer counterfactual rewards at ranks $j \neq k$ for the same item.
% This also means that the IPM requires a strong assumption to ensure full support in the importance weights, i.e.: $\forall a \in \mathcal{A}, x \in \mathcal{X}, k \in [1,L]: \pi(a|x,k) > 0 \implies \pi_{0}(a|x,k) > 0$.

% One structural assumption to alleviate this that is common in the literature comes from the PBM, where we assume that the reward distribution can be factorised as follows:
% \begin{equation}\label{eq:examination_hypothesis}
%     \mathsf{P}(R|X,A,K) = \mathsf{P}(R|X,A) \cdot \mathsf{P}(E|X,K).
% \end{equation}
% Here, $E$ denotes whether an item at position $K$ gets \emph{examined} given context $X$.
% It is aptly known as the \emph{examination hypothesis}~\cite{Craswell2008}, and several works focus on effective and efficient estimation for this term alone~\cite{Fang2019,Jeunen2023_C3PO,Ruffini2022}.
% We will denote estimates for the conditional examination probability $\widehat{\mathsf{P}}(E=1|X=x,K=k)$ as $\rho_{x,k}$.

% This then gives rise to the policy-aware PBM estimator~\cite{Oosterhuis2020,Li2018,gupta2023safe}:
% %
% \begin{equation}
%     \widehat{V}_{\rm PBM}(\pi,\mathcal{D}) =  \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}  r_{k} . 
%     \label{eq:PBM}
% \end{equation}

% \sg{Writing down the estimator and the gradient for PBM in my SIGIR paper's notation for now, I will change it later.}
% %
% \begin{equation}
%     \hat{U}(\pi) = \frac{1}{N} \sum_{i=1}^{N} \sum_{d \in D_{q_i}}  \frac{\rho(d)}{\rho_{0}(d)} c_i(d).
%     \label{cltr-obj}
% \end{equation}
% %
% where the expected exposure $\rho$ is given as:
% \begin{equation}
%     \rho(d \mid q, \pi) =  \mathbb{E}_{y \sim \pi( \cdot \mid q)} \big[ P(E=1 \mid \text{rank}(d \mid y))  \big] = \rho(d).
%     \label{eq:exposurenew}
% \end{equation}

% The gradient of the PBM estimator is given by:
% %
% \begin{equation} 
%       \mathbb{E}_{q, y \sim \pi} \!\mleft[
%       \!\mleft( \sum_{k=1}^K \! \frac{P(E=1 |\, k)}{\rho_{0}(y_k)} \!\mright) \nabla_{\!\pi}\!\log \pi(y) 
%      \!\mright],   
% \end{equation}
% %
% In the gradient estimate, the reward for the log-derivate for a single ranking $y$ is $r(y) = \sum_{k=1}^K \! \frac{P(E=1 |\, k)}{\rho_{0}(y_k)}$. As a baseline for the gradient of the PBM estimator, we propose to use average reward across sampled rankings, i.e. 
% \begin{equation} 
%       \mathbb{E}_{q, y \sim \pi} \!\mleft[
%       \!\mleft( \sum_{k=1}^K \! \frac{P(E=1 |\, k)}{\rho_{0}(y_k)} - \mathbb{E}_{y \sim \pi} \!\mleft( \sum_{k=1}^K \! \frac{P(E=1 |\, k)}{\rho_{0}(y_k)} \!\mright) \!\mright) \nabla_{\!\pi}\!\log \pi(y) 
%      \!\mright],   
% \end{equation}
% % 
% It is clear from the baseline construction that there is a positive covariance between the baseline and the reward for a single sampled ranking, hence the variance of the baseline corrected gradient is lower than it's counterpart without the baseline correction. A similar baseline estimator was used in a recent work on ranking policy training with large language models~\cite{gao2023policy}, and in the context of structured prediction~\cite{kool2019buy}.
% \sg{End of the derivation, mostly borrowed from my previous SIGIR paper notation.}

% If the estimates $\rho_{x,k}$ are unbiased and the examination hypothesis in Eq.~\ref{eq:examination_hypothesis} holds, $\widehat{V}_{\rm PBM}$ is an unbiased estimator of $V(\pi)$.
% Note that the assumption required for full support is weaker than that for the IPM, i.e.: $\forall a \in \mathcal{A}, x \in \mathcal{X}:\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j} > 0 \implies \sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j} > 0$.

% In realistic scenarios, the position bias estimates $\rho_{x,k}$ will lead to a bias--variance trade-off compared to $\widehat{V}_{\rm IPM}$.

% A self-normalised variant of the PBM has not appeared in the research literature.
% One reason for this, is that it is no longer obvious what the control variate should be.
% We explore this further later on.




% \subsubsection{Gradient Calculation with PBM}
% Rewriting the policy-aware policy estimator (Eq.~\ref{eq:PBM}) as:
% %
% \begin{equation}
%     \widehat{V}_{\rm PBM}(\pi,\mathcal{D}) =  \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\rho_{x,a_k,\pi}}{\rho_{x,a_k,\pi_{0}}}  r_{k} . 
% \end{equation}
% %
% where we have substituted the expected exposure as $\sum_{j=1}^{L} \pi(a_{k}|x, j) \\ \rho_{x,j} = \rho_{x,a_k,\pi}$. To estimate the gradient analytically, we focus on a single observation. The gradient for a single observation is given by:
% %
% \begin{equation}
%     \nabla_{\pi} \widehat{V}_{\rm PBM}(\pi,\{x,a,r\}) =  \sum_{k=1}^{L} \frac{\nabla_{\pi} \rho_{x,a_k,\pi}}{\rho_{x,a_k,\pi_{0}}}  r_{k} .
%     \label{eq:PBM-grad}
% \end{equation}
% %
% Focusing on the gradient of the expected exposure term:
% %
% \begin{align}
%     \nabla_{\pi} \rho_{x,a_k,\pi} &= \nabla_{\pi} \mathop{\mathbb{E}}_{a' \sim \pi(. \mid x)}\mleft[ \rho_{x,\mathrm{rank}(a_k \mid a')} \mright] \nonumber \\
%     &= \mathop{\mathbb{E}}_{a' \sim \pi(. \mid x)}\mleft[ \rho_{x,\mathrm{rank}(a_k \mid a')} \nabla_{\pi} \log \pi(a' \mid x) \mright]
% \end{align}
% %
% Substituting it back to Eq.~\ref{eq:PBM-grad} we get:
% %
% \begin{align}
%     \nabla_{\pi} \widehat{V}_{\rm PBM}(\pi,\{x,a,r\}) &= \mleft[ \sum_{k=1}^{L} \mathop{\mathbb{E}}_{a' \sim \pi(. \mid x)} \Big(  \frac{\rho_{x,\mathrm{rank}(a_k \mid a')}}{\rho_{x,a_k,\pi_{0}}}  (r_{k} - b) \Big) \nabla_{\pi} \log \pi(a' \mid x)  \mright]
% \end{align}
% %
% \sg{Sorry for the messy notation, trying different ways here to write down the baseline corrected gradient for the PBM estimator. With a PBM model, we have an expectation term in the gradient, so the variance of this estimator w.r.t the logging policy could be a bit tricky. }
% \oj{Hmm, not straightforward indeed.}
% \sg{Question: The IPS weight used in the PBM estimator $\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}$ is not a function of the logging policy $\pi_0$ anymore, right? Given that we are taking an expectation over all rankings. I am assuming that $\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j} = \mathbb{E}_{a' \sim \pi(. \mid x)} \rho_{x,rank(a_k \mid a')} $.}

% \oj{Not entirely sure what you mean there? Surely it's a function of the logging policy?}

% \sg{We are summing over all possible displayed ranks under the logging policy, so it no longer depends on the logging policy. It's easier to see this from the notation Harrie follows in his top-K paper (Eq 12) \url{https://harrieo.github.io/files/2020-sigir-selection-bias.pdf}. To get the expected exposure under the PBM model, we are marginalizing out the policy $\pi_0$ (summing over all possible rankings under the logging policy.}

% \oj{Trying to derive the gradient below. Is anything wrong in my reasoning?}
% \sg{Removing my previous notation, as it's not consistent with the one we are using here. I was trying to reuse the notation I used in my previous work, and trying to add a baseline and derive the optimal one, but it's not working, so removing it}

% \sg{The difference in notation only comes from the $\pi(a_k \mid x, k)$ term. I just expanded it in terms of expectation over all rankings. I am assuming $\pi(a \mid x, k) = \mathop{\mathbb{E}}_{A \sim \pi(\cdot|x)} ( \mathbbm{1}(A_k = a) ) $. Does that make sense? }

% The gradient for the PBM estimator is given by:
% \begin{align}
%     \nabla(V_{\rm PBM}(\pi)) &=  \nabla\mleft( \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi(\cdot|x)}\mleft[ \sum_{k=1}^{L} r_{k} \mright]\mright] \mright)\nonumber\\ 
%     &=  \nabla\mleft( \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot|x)}\mleft[  \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} r_{k} \mright]\mright] \mright)\nonumber\\    
%     &=  \nabla\mleft(\int\sum_{a \in \mathcal{A}} \pi_{0}(a|x)  \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} r_{k}\mathsf{P}(X=x)\rm{d}x \mright) \nonumber\\
%     &=  \int\sum_{a \in \mathcal{A}} \pi_{0}(a|x)  \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\nabla\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} r_{k}\mathsf{P}(X=x)\rm{d}x \nonumber\\   
%     &=  \mathop{\mathbb{E}}_{x\sim\mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot|x)}\mleft[  \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\nabla\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} r_{k} \mright]\mright].
% \end{align}

% This allows for Monte Carlo estimation and baseline corrections, analogously to the other estimators presented throughout this work.

% \subsection{Self-Normalisation in the PBM}
% \oj{This Section is messy, unfinished, and of limited interest.}

% \textcolor{Maroon}{\tt TODO: derive, analogously to SNIPM, a control variate that allows for self-normalisation of $\widehat{V}_{\rm PBM}$.}

% The control variates for SNIPS/SNIPM(-G) are simply quantities with a known expectation that also correlate with the IPS/IPM estimator, which then reduces the variance of the \emph{self-normalised} IPS/IPM estimators.
% If these control variates correlate with the PBM estimator, we could directly apply them to obtain a self-normalised PBM variant.
% Note that this might not provide optimal variance reduction---if we can devise a PBM-centric control variate with a stronger correlation, this would be preferable.
% Additionally, as we will show further on, simply repurposing the SNIPM control variate does not allow us to deduce an equivalence between self-normalisation and reward translation.

% SNIPS leverages the average importance weight from the IPS estimator, and SNIPM analogously leverages the average importance weight under the IPM estimator.
% As such, it is natural to define a control variate for the PBM estimator as:
% \begin{equation}\label{eq:control_variate_pbm}
% \begin{split}    
%    \mathop{\mathbb{E}}_{(x,a,r) \sim \mathsf{P}(X,A,R|\Pi=\pi)}\mleft[
%    \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}}\sum_{k=1}^{L}\frac{\sum_{j=1}^{L} \pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L} \pi_{0}(a_{k}|x, j) \rho_{x,j}}
%    \mright]\\
%   = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot |x)}\mleft[\sum_{k=1}^{L}
%     \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}
%   \mright]\mright]\\
%   = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[ \sum_{a \in \mathcal{A}} \sum_{k=1}^{L} \pi_{0}(a_{k}|x, k) 
%     \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}
%   \mright]\\
% %   = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[ \sum_{a \in \mathcal{A}} \sum_{k=1}^{L}
% %    \sum_{j=1}^{L}  \pi_{0}(a_{k}|x, k) \frac{\pi(a_{k}|x, j) \rho_{x,j}}{\pi_{0}(a_{k}|x, j) \rho_{x,j}}
% %   \mright]\\
% %   = \mathop{\mathbb{E}}_{(x,a,r) \sim \mathsf{P}(X,A,R|\Pi=\pi)}\mleft[
% %    \sum_{k=1}^{L} \sum_{j=1}^{L} \frac{\pi(a_{k}|x, j) \rho_{x,j}}{\pi_{0}(a_{k}|x, j) \rho_{x,j}}
% %   \mright]\\
%    \stackrel{?}{=} ?.
% \end{split}
% \end{equation}
% Nevertheless, it is unclear what this expectation amounts to, at this point. Can we somehow estimate its expectation?

% \textcolor{Maroon}{\tt TODO: I was so far unable to actually show that this will equal 1 and be a sensible control variate. Is it?}
% % \sg{I tried to prove it but was unable to do so as well. But does the control variate have to be equal to 1 in expectation necessarily? In the BanditNet paper (as far as I remember), this property was used to restrict the search space of the $\lambda$ hyperparam around 1. For the PBM user model, we can come up with a different way to tune the $ \lambda $ in case the control variate doesn't come out to be $ 1 $ in expectation. I'll read up a bit more on multiplicative control variates to be sure.}

% % Intuitively, this control variate represents the average exposure allocated to items.
% % Following the assumptions of the PBM, this is entirely determined by $\rho_{x,j}$ and cannot be influenced by any $\pi$, so the ratio must equal 1.
% % \textcolor{Maroon}{Right?}
% % \textcolor{Maroon}{Note: Ben London mentioned that Thorsten Joachims \& co. have been considering similar extensions, but that Thorsten is convinced this doesn't make sense. I don't really know why though.}
% This then gives rise to a new estimator:
% \begin{equation}
%     \widehat{V}_{\rm SNPBM}(\pi, \mathcal{D}) =  \frac{\sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L}  \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}  r_{k}   }{\sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}}.
% \end{equation}


% \subsubsection{Shenanigans to get a sensible control variate}
% Suppose we assume that $\rho_{x,j} \perp \!\!\! \perp j | x$.
% That is, $\mathsf{P}(E=1|X=x,K=j)\equiv\mathsf{P}(E=1|X=x)\equiv \rho_{x}$ Now:
% \begin{equation}
% \begin{split}    
%    \mathop{\mathbb{E}}_{(x,a,r) \sim \mathsf{P}(X,A,R|\Pi=\pi)}\mleft[
%    \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}}\sum_{k=1}^{L}\frac{\sum_{j=1}^{L} \pi(a_{k}|x, j) \rho_{x}}{\sum_{j=1}^{L} \pi_{0}(a_{k}|x, j) \rho_{x}}
%    \mright]\\
%     = \mathop{\mathbb{E}}_{(x,a,r) \sim \mathsf{P}(X,A,R|\Pi=\pi)}\mleft[
%    \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}}\sum_{k=1}^{L}\frac{\rho_{x} \sum_{j=1}^{L} \pi(a_{k}|x, j)}{\rho_{x}\sum_{j=1}^{L} \pi_{0}(a_{k}|x, j)}
%    \mright]\\
%     = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot |x)}\mleft[\sum_{k=1}^{L}
%     \frac{\rho_{x}\sum_{j=1}^{L}\pi(a_{k}|x, j)}{ \rho_{x}\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) }
%   \mright]\mright]\\
%     = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot |x)}\mleft[\sum_{k=1}^{L}
%     \frac{\rho_{x} \cdot 1}{ \rho_{x} \cdot 1 }
%   \mright]\mright]\\
%     = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot |x)}\mleft[ L
%   \mright]\mright]\\
%   = L.
% \end{split}
% \end{equation}
% This feels rather useless.

% Even if we do not find a clean simplification of this expectation, can we just write out its analytical form and use this to normalise?
% This probably means we need to be able to write out the entire logging and target policies, i.e. every $\pi(a|x,j)$ combination.
% But I guess that can be acceptable if we only need to do this once?

% \begin{equation}
% \begin{split}    
%    \mathop{\mathbb{E}}_{(x,a,r) \sim \mathsf{P}(X,A,R|\Pi=\pi)}\mleft[
%    \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}}\sum_{k=1}^{L}\frac{\sum_{j=1}^{L} \pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L} \pi_{0}(a_{k}|x, j) \rho_{x,j}}
%    \mright]\\
%   = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[\mathop{\mathbb{E}}_{a \sim \pi_{0}(\cdot |x)}\mleft[\sum_{k=1}^{L}
%     \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}
%   \mright]\mright]\\
%   = \mathop{\mathbb{E}}_{x \sim \mathsf{P}(X)}\mleft[ \sum_{a \in \mathcal{A}}\sum_{k=1}^{L} \pi_{0}(a_{k}|x, k)
%     \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}
%   \mright]\\
%   = \int \mathsf{P}(X=x) \sum_{a \in \mathcal{A}}\sum_{k=1}^{L} \pi_{0}(a_{k}|x, k)
%     \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} {\rm d}x
% \end{split}
% \end{equation}

% \sg{We can test this out with the simple top-1 off-policy BanditNet setup (Eq 10). If we substitute $\lambda$ in Eq. 10 with the average IS ratio (denominator from SNIPS), and if optimizing for it improves upon the constant $\lambda$ objective, then we can show that avg. empirical importance ratio weights can also help with reducing the variance. If that works out we can use the average IS ratio (denominator in Eq 20) as control variate for PBM model. Does that make sense? We can also use the running average of the average IS ratio across the mini-batches during the training as a  baseline.}


% \sg{In the simple top-1 recommendation setup Eq.3)}, if we use the average IS ratio as a baseline correction, then we can work backwards from the lagrangian formulation to the SNIPS objective, since we are setting $\lambda$ exactly as $S$ in this case, from the BanditNet formulation. It is a valid value for $\lambda$ since the paper assumes a monotonic relation between $\lambda$ and $S$ (Theorm 1, Appendix A, BanditNet).

% \begin{equation}
% \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}}\frac{\pi(a|x)}{\pi_{0}(a|x)}
% \end{equation}

% \sg{TODO: Assuming this value of the $\lambda$, work backwards to show that this is equivalent to optimizing for the SNIPS estimator. If this works out correct, we can use this value in the BanditNet framework, which is equivalent to optimizing for the SNIPS estimator, and that the $\lambda$ is not constraint to be equal to 1 in expectation.}
% If we set this value for $\lambda$, there is also a connection between the new $\lambda$ translated reward objective and the POEM objective. \sg{This statement is not correct when I tried writing down the proof. I was trying to connect the average IS ratio to the variance of the estimator, but it's not connected}

% \sg{Does this make sense? If this works out correct, then we have to prove the same for the PBM model, and then just use the average IS term (Eq. 19) as a baseline.}

% \subsection{Self-Normalisation via Reward Translation}\label{sec:SNIPM_reward_translation}
% As discussed in Section~\ref{sec:general_OPE}, \citeauthor{Joachims2018} show that a policy optimised for SNIPS (which is unachievable by standard mini-batch optimisation techniques) can be learned by optimising for IPS with a translation on the reward instead~\cite{Joachims2018}.
% We have shown that this practice is equivalent to applying a baseline correction, designed to combat variance in the gradient of the IPS estimator.

% In what follows, we derive equivalent analogues for SNIPM(-G).
% The derivations heavily draw from~\cite[\S 3.3]{Joachims2018}.
% These results emphasise that the BanditNet insight extends to ranking problems, allowing for efficient optimisation of off-policy learning approaches for self-normalised estimators in ranking settings.
% Similar to BanditNet, the translation $\lambda$ should be seen as a hyper-parameter to be tuned accordingly, either via grid search or more sophisticated approaches.
% Moreover, the insight that these approaches can be linked to baseline corrections, extends to rankings as well.


% \subsubsection{SNIPM-G}
% Define the optimisation problem:
% \begin{gather}    
%     \pi^{\star} = \argmax_{\pi \in \Pi} \widehat{V}_{\rm SNIPM-G}(\pi, \mathcal{D}),\nonumber\\
%     \text{ with } S^{\star} = \frac{1}{\mleft|\mathcal{D}\mright|}\sum_{(x,a,r) \in \mathcal{D}} \frac{1}{L}\sum_{k=1}^{L} \frac{\pi^{\star}(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)}.
% \end{gather}
% This is equivalent to the constrained optimisation problem:
% \begin{gather}
%     \pi^{\star} = \argmax_{\pi \in \Pi} \widehat{V}_{\rm IPM}(\pi, \mathcal{D}), \nonumber\\
%     \text{s. t. } \frac{1}{\mleft|\mathcal{D}\mright|}\sum_{(x,a,r) \in \mathcal{D}} \frac{1}{L} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} = S^{\star}.
% \end{gather}
% Consider the Lagrangian for this constrained optimisation problem:
% \begin{align}\label{eq:lagrangian}
%     L(\pi,\lambda) = &\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} r_{k} \nonumber\\
%     &\quad - \lambda \mleft[\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \frac{1}{L} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} - S^{\star}\mright] \nonumber\\
%     = &\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} (r_{k}-\frac{\lambda}{L})+\lambda S^{\star}.
% \end{align}
% This shows that optimising SNIPM-G can be achieved by optimising IPM with a translation on the reward, instead:
% \begin{gather}
%     \pi^{\star} =  \argmax_{\pi \in \Pi} \widehat{V}_{\lambda^{\star}-{\rm IPM}}(\pi, \mathcal{D}), \text{where }\nonumber\\ 
%     \widehat{V}_{\lambda-{\rm IPM}}(\pi,\mathcal{D}) = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} (r_{k}-\lambda).
% \end{gather}

% \subsubsection{SNIPM}
% Define the optimisation problem:
% \begin{gather}    
%     \pi^{\star} = \argmax_{\pi \in \Pi} \widehat{V}_{\rm SNIPM}(\pi, \mathcal{D}),\nonumber\\
%     \text{ with } S_{k}^{\star} = \frac{1}{\mleft|\mathcal{D}\mright|}\sum_{(x,a,r) \in \mathcal{D}}\frac{\pi^{\star}(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)}, \forall  k \in [1,L].
% \end{gather}
% This is equivalent to the constrained optimisation problem:
% \begin{gather}
%     \pi^{\star} = \argmax_{\pi \in \Pi} \widehat{V}_{\rm IPM}(\pi, \mathcal{D}),\nonumber\\
%     \text{s. t. } \frac{1}{\mleft|\mathcal{D}\mright|}\sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} = S_{k}^{\star}, \forall k \in [1,L] .
% \end{gather}
% Consider the Lagrangian for this constrained optimisation problem, where $\lambda_k$ denotes the Lagrange multiplier for constraint $S_{k}^{\star}$:
% \begin{align}
%     L(\pi,\lambda) = &\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} r_{k} \nonumber\\
%     &\quad - \sum_{k=1}^{L}\lambda_{k} \mleft[\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} - S_{k}^{\star}\mright] \nonumber\\
%     = &\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} (r_{k}-\lambda_{k})+ \sum_{k=1}^{L}\lambda_{k} S_{k}^{\star}.
% \end{align}
% \textcolor{Maroon}{I think the derivation is correct, but should be checked properly.}

% This shows that optimising SNIPM can be achieved by optimising IPM with a translation on the reward, instead.
% Contrary to SNIPM-G where the $\lambda$ is \emph{global}, this translation is position-specific or \emph{local}:
% \begin{gather}
%     \pi^{\star} =  \argmax_{\pi \in \Pi} \widehat{V}_{\lambda_{k}^{\star}-{\rm IPM}}(\pi, \mathcal{D}), \text{where } \nonumber\\ 
%     \widehat{V}_{\lambda_{k}-{\rm IPM}}(\pi,\mathcal{D}) = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\pi(a_{k}|x, k)}{\pi_{0}(a_{k}|x, k)} (r_{k}-\lambda_{k}).
% \end{gather}

% \textcolor{Maroon}{Quite interesting that the local variant allows for more flexibility on the translation. Can we make $\lambda$ dependent on more information? $\lambda(k,x)$? Is that even sensible?}

% \sg{BanditNet objective (similar to SNIPM-G) was also used with slates (rankings) in a AAAI 2018 paper~\cite{lopez2021learning} }

% \subsubsection{SNPBM}
% Define the optimisation problem:
% \begin{gather}    
%     \pi^{\star} = \argmax_{\pi \in \Pi} \widehat{V}_{\rm SNPBM}(\pi, \mathcal{D}),\nonumber\\
%     \text{ with } S^{\star} = \frac{1}{\mleft|\mathcal{D}\mright|}\sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi^{\star}(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}.
% \end{gather}
% This is equivalent to the constrained optimisation problem:
% \begin{gather}
%     \pi^{\star} = \argmax_{\pi \in \Pi} \widehat{V}_{\rm PBM}(\pi, \mathcal{D}), \nonumber\\
%     \text{s. t. } \frac{1}{\mleft|\mathcal{D}\mright|}\sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} = S^{\star}.
% \end{gather}
% Consider the Lagrangian for this constrained optimisation problem:
% \begin{align}
%     L(\pi,\lambda) = &\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} r_{k} \nonumber\\
%     &\quad - \lambda \mleft[\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}}  - S^{\star}\mright] \nonumber\\
%     = &\frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} (r_{k}-\lambda)+\lambda S^{\star}.
% \end{align}
% This shows that optimising SNPBM can be achieved by optimising PBM with a translation on the reward, instead:
% \begin{gather}
%     \pi^{\star} =  \argmax_{\pi \in \Pi} \widehat{V}_{\lambda^{\star}-{\rm PBM}}(\pi, \mathcal{D}), \text{where }\nonumber\\ 
%     \widehat{V}_{\lambda-{\rm PBM}}(\pi,\mathcal{D}) = \frac{1}{\mleft|\mathcal{D}\mright|} \sum_{(x,a,r) \in \mathcal{D}} \sum_{k=1}^{L} \frac{\sum_{j=1}^{L}\pi(a_{k}|x, j) \rho_{x,j}}{\sum_{j=1}^{L}\pi_{0}(a_{k}|x, j) \rho_{x,j}} (r_{k}-\lambda).
% \end{gather}

% \subsection{Baseline Corrections Imply Self-Normalisation}
% \textcolor{Maroon}{\tt TODO: discuss how recent counterfactual LTR work performs baseline corrections on gradient estimates, to reduce variance. Discuss how this is equivalent to the approach described in 3.2.}

% \citeauthor{Joachims2018} discuss this briefly near the end of Section 3~\cite{Joachims2018}, stating: ``\textit{it is unclear whether gradient variance, as opposed to variance of the ERM objective, is really the key issue in batch learning from bandit feedback}''.
% Not sure how this translates to our setting, yet.
% % \sg{Maybe we can analytically (or empircally) compare the variance of the gradient with different estimators?}

%%%%%%%% A random idea for a short paper maybe?
% \sg{Just a random idea for a short paper, writing it down here for later.}
% \sg{With the SNIPS estimator, Can't we take a log of the original estimator $log_{E(f)/E(G)}$ and then apply Jensen's to move the log inside the expectation? It will be an lower (or upper, forgot the direction of Jensens') bound on the original objective, but for learning purpose, it should work (since we can replace expectation with sample? \citet{liang2022local} do something along this line.}

% \begin{align}
%     \log\mleft(\frac{\mathbb{E}[\frac{\pi(a \mid x)}{\pi_{0}(a \mid x)}r(a,x)]}{\mathbb{E}[\frac{\pi(a \mid x)}{\pi_{0}(a \mid x)}]}\mright) \geq \mathbb{E}\mleft( \log \mleft[\frac{\frac{\pi(a \mid x)}{\pi_0(a \mid x)} r(a, x)}{\frac{\pi(a \mid x)}{\pi_0(a \mid x)}} \mright] \mright)
% \end{align}
% Second step is the application of Jensen's inequality. 
% This results in the following lower-bound on the SNIPS estimator:
% \begin{align}
%     &\mathbb{E}\mleft( \log \mleft[\frac{\pi(a \mid x)}{\pi_0(a \mid x)} r(a, x) \mright] \mright) - \mathbb{E}\mleft( \log \mleft[\frac{\pi(a \mid x)}{\pi_0(a \mid x)} \mright] \mright) \\
%     &\approx 
% \end{align}
% %
% \sg{Boils down to a weighted log-likelihood with a KL-divergence constraint? When is the lower-bound tight? }
%%%%%%%%%%

\oj{Very rough idea: Effective Sample Size is a common diagnostic for IPS estimators. Owen's book provides a formula for the ESS that depends on the reward~\cite[Eq. 9.17]{Owen2013}. What if we aim to use a baseline that maximises the ESS? Would this be equivalent to minimising variance? I'll try to take some time to check.
Maximising effective sample size boils down to minimising the coefficient of variation of the weights (see ~\cite[Eq. 9.15]{Owen2013}).
As such, if we can show that our baseline minimises this value, we're done.
Coefficient of variation is defined as standard-deviation over mean for the weights. In our case, these are~\cite[Eq. 9.17]{Owen2013}:
}
\begin{equation}
    w_{i} = \frac{\frac{\pi(a_{i}|x_{i})}{\pi_{0}(a_{i}|x_{i})} | r_{i}-\beta |}{\sum_{j} \frac{\pi(a_{j}|x_{j})}{\pi_{0}(a_{j}|x_{j})} | r_{j}-\beta |}
\end{equation}
As Owen writes, the CoV is then:
\begin{equation}
    {\rm cv}(w) = \sqrt{n\sum_{i=1}^{n}(w_{i}^{2}) - 1}
\end{equation}
What is the value of $\beta$ that minimises this quantity?op



%%%%%%%%
% related to comments about baseline correction from the BanditNet paper.
% Indeed, this quantity can simply be estimated from the logged dataset we learn from.

% \oj{TODO: check with Thorsten? Maarten is also an author of that paper. What do you think?}
% \sg{I will check with Maarten, but if you could also ask Thorsten, that would be great.}
% \oj{(E-mailed Thorsten)}
% \sg{Thanks :).}


% \sg{Do you think it makes sense to run this analysis again with more practical estimators and optimizers. For ex: with clipped IPS and with Adam optimizer? I don't think I have seen many papers analysing the gradients of the IPS objective when using more advanced (and practical) optimizer like Adam, RMSProp etc. Or is this not interesting for a research paper and more of a practical question? I was just wondering what would the gradient updates look like if we plug in the IPS gradient with optimal baseline into Adam/RMSpro etc.}

% \sg{A practical thing to consider: if we use a stochastic sample estimate of the optimal baseline, it it not unbiased(?), given we have a ratio of expectations (similar to SNIPS). So if we were to use a sample estimate of the optimal baseline, what is the bias of the resulting estimator?}

% \oj{Definitely an interesting question. I suppose it's asymptotically unbiased in the same way that SNIPS is?}

% \oj{Reference to figure out bias and variance of the estimate: ~\cite[Eq. 2.30, 2.33]{Owen2013} at \href{https://artowen.su.domains/mc/Ch-intro.pdf}{this url}}
% \sg{The variance of the sample estimate of the optimal baseline goes down at the rate of $\mathcal{O}(\frac{1}{N^2})$, and the bias goes down at the rate of $\mathcal{O}(\frac{1}{N})$ (~\cite[Eq. 2.30--2.32]{Owen2013} at \href{https://artowen.su.domains/mc/Ch-intro.pdf}{this url}, so we might either need to use very large batch-size, or use a full-batch GD. I am trying to setup an experiment to test it out empirically. }

%%%
% related to the application of log-derivative trick in the off-policy estimator.

% \oj{Thank you for this! I changed things slightly because it seems simpler to only consider $\frac{\nabla \pi}{\pi_{0}}$, not bothering with the log-trick when it isn't strictly necessary. Kept yours in comment so we can discuss if you disagree.}
% \sg{This is the variance optimal baseline for off-policy bandits. The expectation is over the actions from the logging policy $\pi_0$, so it can be easily estimated from the logged data. I am not sure why existing off-policy learning methods don't use this as a baseline. Do you think the derivation makes sense? Maybe I missed some step, because this looks pretty simple to plug in to existing estimators.}

% \oj{I don't see why it wouldn't work, at first glance... Might make sense to have someone (like Ben, Harrie or Maarten) check the derivation, but this looks great to me.}

% \sg{Connection to SNIPS: Given this is the 'optimal' baseline, the BanditNet's (or any other baseline correction for that matter) policy gradient variance should be higher than this, right? The variance is a convex function of 'b', so the optimal baseline we derive should be the global minimum. Now I am not sure of any direct relation between $b^{*}$, and $S^{*}$ (SNIPS). What do you think?}

% \oj{I agree. It would be "cool" if we could somehow work back to find the value of $S^{\star}$ that matches this optimal baseline, but not strictly necessary for things to be useful.}

% \sg{If we can derive something similar for the PBM model, this itself could be a contribution? Does the baseline really have to be related to the SNIPS estimator? We can use the SNIPS/BanditNet estimator as a baseline, with a constant (tunable) baseline correction. We can also analyse the variance of the policy-gradient for the BanditNet estimator. The $\lambda$ used in inspired from the multiplicative control variate used in SNIPS, but in practice it is treated as a hyper-parameter, hence a constant, so the variance of the gradient of the BanditNet estimator should be same as the variance of the IPS estimator?.}
% \oj{Why would the variance of the gradient of BanditNet equal the variance of the gradient of IPS? It depends on the $\lambda$ (i.e. $\beta$) value, right?}
% \sg{Right, in theory, yes, it depends on $\beta$, but in practice, it is treated as a hyper-parameter, with a hyper-parameter search range around 1. But an implementation detail, so I got a bit confused. This is not a major point, we can ignore it.}



% \sg{BanditNet requires a tuning of the $\lambda$ parameter, whereas with our optimal baseline, it requires no parameter tuning, and in theory has a lower variance as compared to BanditNet, this should be make a good selling point?}





%%%%%%%%%%%%%%%%%

% Intro comments
% \oj{I'll write an intro with this structure}
% \begin{enumerate}
%     \item Recommender systems are moving towards the decision-making paradigm
%     \item Within this area, all works showing strong online performance are actually off-policy
%     \item Variance is an issue for off-policy methods. Rich literature exists.
%     \item We draw connections, highlight the equivalence (for learning), and derive the optimal baseline
%     \item Experiments show we rock
% \end{enumerate}


% ----------------~\\
% The current draft roughly follows this structure:
% \begin{enumerate}

%     \item Introduce on-policy contextual bandits
%     \begin{enumerate}
%         \item Focus on policy gradients, i.e. REINFORCE

%         \item Talk about control variates:
%         \begin{enumerate}
%             \item Additive control variate to reduce variance of gradient (i.e. baseline correction)
%             \item Additive control variate to reduce variance of estimator (i.e. ``regression adjustment'')
%         \end{enumerate}
%     \end{enumerate}

%     \item Introduce off-policy contextual bandits
%     \begin{enumerate}
%         \item Focus on IPS
%         \item Talk about control variates
%         \begin{enumerate}
%             \item Additive control variate to reduce variance of gradient (i.e. baseline correction)
%             \item Additive control variate to reduce variance of estimator (i.e. ``regression adjustment'') -- this is doubly robust.
%             \item Multiplicative control variate to reduce variance of estimator -- this is self-normalisation.
%             \item Reduction from SNIPS to BanditNet, highlighting that all of the above are similar in spirit. (Highlight that $\lambda$ in BanditNet $=V_{\rm SNIPS}$)
%             \item Derivation of the optimal (variance-minimising) baseline correction.

%         \end{enumerate}
%     \end{enumerate}
%     \item Introduce off-policy learning-to-rank ~\cite{Joachims2017}
%     \begin{itemize}
%         \item IPM -- not using estimated position biases ~\cite[\S 3.2]{Li2018}
%         \begin{enumerate}
%             \item For IPM, we can reiterate all-of-the-above and show how the equivalence extends
%         \end{enumerate}
%         % \item PBM -- using estimated position biases ~\cite[\S 3.5]{Li2018}
%         % \begin{enumerate}
%         %     \item For PBM, we do not have self-normalisation (multiplicative CV is unclear). Can we work backwards from Harrie's DR formulation?
%         % \end{enumerate}
%         \sg{Removing the PBM stuff for now.}
%     \end{itemize}
% \end{enumerate}


%%% Discussion experimental setup
% \sg{Ran experiments on openbandit fully synthetic setup. Results are as expected, beta-IPS has lower MSE than even the DR estimator (surprising), but the SNIPS method almost exactly overlaps with the Beta-IPS estimator, which is strange.}
%     \sg{Should we keep both results? One results for the the continuous setting, and the other one for the discrete setting. }
%     \oj{Very surprising that we can do better than DR, what is the reward model in this case? I guess the synthetic OBP setting might favour SNIPS: if the optimal baseline is close to SNIPS, then they will become equivalent. But SNIPS doesn't have guarantees, and we do. When will SNIPS start to break down?}
%     \sg{Yeah, the comparision with DR is surprising. The reward/regression model is  a logistic regression model. Could that be a problem? I  will try with a GDBT model. }

%     \oj{If the reward isn't linear, it might be. This relates to the MRDR paper~\cite{Farajtabar2018}: a reward model optimised to minimise the variance of the overall estimator can be better than a more accurate model. I think this can be a nice result showcasing that DR isn't always a silver bullet. (See ~\cite{Jeunen2020REVEAL} for a very basic similar experiment)}


%     \sg{I think I found the issue with the synthetic setup which resulted in an overlap b/w SNIPS and beta-IPS. The average reward in the synthetic dataset is relatively high (around 0.6), which results in the optimal baseline to be close to $1$ most of the times, resulting in a similar behavior as the SNIPS estimator (numerator and denominator overlap). I ran an experiment with a sparse reward function and now it seems like SNIPS and beta-IPS are diverging :)}

%     \oj{Let's try to add this intuition to the text somewhere (I don't want to cherry-pick results), but it feels like this setting is more realistic! We could try to pick a stronger regression model for DM/DR too, but this is starting to look really nice :) thanks Shashank!}
